The Fact Selection Problem in LLM-Based Program Repair

Recent research has shown that incorporating bug-related facts, such as stack traces and GitHub issues, into prompts enhances the bug-fixing capabilities of large language models (LLMs). Considering the ever-increasing context window of these models, a critical question arises: what and how many facts should be included in prompts to maximise the chance of correctly fixing bugs? To answer this question, we conducted a large-scale study, employing over 19K prompts featuring various combinations of seven diverse facts to rectify 314 bugs from open-source Python projects within the BugsInPy benchmark. Our findings revealed that each fact, ranging from simple syntactic details like code context to semantic information previously unexplored in the context of LLMs such as angelic values, is beneficial. Specifically, each fact aids in fixing some bugs that would remain unresolved or only be fixed with a low success rate without it. Importantly, we discovered that the effectiveness of program repair prompts is non-monotonic over the number of used facts; using too many facts leads to subpar outcomes. These insights led us to define the fact selection problem: determining the optimal set of facts for inclusion in a prompt to maximise LLM's performance on a given task instance. We found that there is no one-size-fits-all set of facts for bug repair. Therefore, we developed a basic statistical model, named Maniple, which selects facts specific to a given bug to include in the prompt. This model significantly surpasses the performance of the best generic fact set. To underscore the significance of the fact selection problem, we benchmarked Maniple against the state-of-the-art zero-shot, non-conversational LLM-based bug repair methods. On our testing dataset of 157 bugs, Maniple repairs 88 bugs, 17% above the best configuration.

==> sections/future_work.tex <==
\section{Future Work}
\label{sec:future}
Our current work provides a proof of concept for a successful dynamic fact selection strategy by providing a simple model which performs better than the best static fact selection strategy on our dataset. There is a substantial potential for further refinement. Our next steps involve constructing a more robust dynamic fact selection strategy and benchmarking it against the established feature selection techniques used within the machine learning landscape.

 In this work, we treated Large Language Models (LLMs) as black boxes, focusing on leveraging their capabilities for prompt generation without delving into their internal workings. However, a promising avenue for future exploration lies in fine-tuning LLMs for prompt refinement. This approach could enable the automatic generation of even better prompts specifically tailored for program repair tasks, potentially leading to further improvements in repair effectiveness.
 
Additionally, our observations highlight a challenge with Large Language Models (LLMs) — performance drops when the prompts are too long. Preliminary analysis of our dataset indicates a clear correlation between prompt length and pass@1 scores, as we've detailed in \cref{sec:maniple:select}. This insight has not only motivated the incorporation of prompt length as a critical feature in our random forest classifier but also sheds light on the non-monotonicity with respect to the number of facts, as adding more facts will increase the prompt length. Consequently, the development of sophisticated prompt compression techniques emerges as a promising avenue for research, poised to significantly enhance the performance of LLMs by distilling essential information into more concise, potent prompts. 

\sergey{few-shot approach}

In our present study, we've limited our interaction with the Large Language Model (LLM) to a single query. However, the realm of fully automated, dialogue-based program repair strategies holds considerable promise. Such approaches could transform fact selection into a dynamic, iterative process, engaging LLM in a series of queries. Frameworks like ReACT, as mentioned in Yao et al.~\cite{yao2022react}, provide a blueprint for how LLMs can actively seek specific information from a repository, using this to reason through and ultimately resolve the bug. Such multi prompt methods open up new avenues for leveraging LLM capabilities.
\sergey{multi-prompt/toolformer/augmented llm}


